A Priori Error Bounds for the Approximate Deconvolution Leray Reduced Order Model

The approximate deconvolution Leray reduced order model (ADL-ROM) uses spatial filtering to increase the ROM stability, and approximate deconvolution to increase the ROM accuracy. In the under-resolved numerical simulation of convection-dominated flows, ADL-ROM was shown to be significantly more stable than the standard ROM, and more accurate than the Leray ROM. In this paper, we prove a priori error bounds for the approximate deconvolution operator and ADL-ROM. To our knowledge, these are the first numerical analysis results for approximate deconvolution in a ROM context. We illustrate these numerical analysis results in the numerical simulation of convection-dominated flows.

==> notation.tex <==
% environments
\makeatletter
\@ifclassloaded{article}{  % preprint format
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{algorithmplain}{Algorithm}[section]
}{ % journal format
\theoremstyle{thmstyletwo}%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}%
\newtheorem{lemma}[theorem]{Lemma}%
\newtheorem{assumption}{Assumption}%
\newtheorem{example}{Example}%
\newtheorem{remark}{Remark}%
\newtheorem{definition}{Definition}
\newtheorem{algorithmplain}{Algorithm}
\numberwithin{equation}{section}
}
\makeatother

% For some reason the journal format does not render \boldsymbol in bold.
% Use the macros below for boldface letters.
% Undefine it to make sure that \boldsymbol does not creep in again.
% Do the same for overline for consistency
\let\boldsymbol\undefined
\let\overlineIMPLEMENTATION\overline
\let\overline\undefined

% boldface Greek letters
\newcommand{\bfeta}{\pmb{\eta}}
\newcommand{\bPhi}{\pmb{\Phi}}
\newcommand{\bphi}{\pmb{\phi}}
\newcommand{\bvarphi}{\pmb{\varphi}}

% boldface letters
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bX}{\mathbf{X}}

% boldface numbers
\newcommand{\bzero}{\mathbf{0}}

% overline letters
\newcommand{\obu}{\overlineIMPLEMENTATION{\bu}}
\newcommand{\obullet}{\overlineIMPLEMENTATION{\bullet}}
\newcommand{\obphi}{\overlineIMPLEMENTATION{\bphi}}
\newcommand{\obuk}[1]{\overlineIMPLEMENTATION{ \bu_{#1}}}
\newcommand{\obfetak}[1]{\overlineIMPLEMENTATION{ \bfeta_{#1}}}
\newcommand{\oburk}[2][r]{\overlineIMPLEMENTATION{ \bu_{#2}^{#1}}}
\newcommand{\obPhirk}[2][r]{\overlineIMPLEMENTATION{ \bu_{#2}^{#1}}}

% comments
\begin{comment}
\definecolor{vargreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\ti}[1]{{\color{blue}TI: #1}}
\newcommand{\fb}[1]{{\color{vargreen}FB: #1}}
\newcommand{\im}[1]{{\color{brown}IM: #1}}
\newcommand{\asf}[1]{{\color{purple}AS: #1}}
\newcommand{\rev}[1]{{\color{blue}#1}}
\end{comment}
